Large batch size training of neural networks with adversarial training and second-order information

The most straightforward method to accelerate Stochastic Gradient Descent (SGD) computation is to distribute the randomly selected batch of inputs over multiple processors. To keep the distributed processors fully utilized requires commensurately growing the batch size. However, large batch training often leads to poorer generalization. A recently proposed solution for this problem is to use adaptive batch sizes in SGD. In this case, one starts with a small number of processes and scales the processes as training progresses. Two major challenges with this approach are (i) that dynamically resizing the cluster can add non-trivial overhead, in part since it is currently not supported, and (ii) that the overall speed up is limited by the initial phase with smaller batches. In this work, we address both challenges by developing a new adaptive batch size framework, with autoscaling based on the Ray framework. This allows very efficient elastic scaling with negligible resizing overhead (0.32\% of time for ResNet18 ImageNet training). Furthermore, we propose a new adaptive batch size training scheme using second order methods and adversarial training. These enable increasing batch sizes earlier during training, which leads to better training time. We extensively evaluate our method on Cifar-10/100, SVHN, TinyImageNet, and ImageNet datasets, using multiple neural networks, including ResNets and smaller networks such as SqueezeNext. Our method exceeds the performance of existing solutions in terms of both accuracy and the number of SGD iterations (up to 1\% and $5\times$, respectively). Importantly, this is achieved without any additional hyper-parameter tuning to tailor our method in any of these experiments.

==> algo.tex <==
\begin{algorithm}
\DontPrintSemicolon
\caption{Algorithm needs to be fixed: Adaptive Batch Size (ABS) and Adaptive Batch Size Adversarial (ABSA)}\label{alg:abs}
   \SetAlgoLined
    \KwInput{Learning rate $\eta$, decay epoch $E_{decay}$, decay ratio $\rho_{lr, decay}$; initial batch $B_{init}$, maximum batch $B_{max}$; Eigenvalue decay ratio $\alpha$, batch/lr increasing ratio $\beta$, duration factor $\kappa$; adversarial input ratio $\gamma$, adversarial magnitude $\epsilon_{adv}$, adversarial input ratio decay factor $\omega$, terminate epoch $\tau$; input data $x$. }
    \KwResult{Final model parameters $\theta$}
    Initialize old (new) eigenvalue as $\lambda_{old}$ ($\lambda_{new}$), batch size $B_{itr}$, learning rate $\eta_{itr}$, duration time $\kappa_{itr}=0$.
    
    \For{Epoch $=1,2,3\ldots$}{
      \For(\tcp*[h]{mini-batch iterations}){$t=1,2,3\ldots$}{
        generate adversarial data $x_{adv}$ by the ratio of $\gamma$;
        
        SGD update;
      }
     
      compute $\lambda_{new}$; \tcp*[h]{Hessian power-iteration}
      
      $\kappa_{itr} \pluseq 1$;
      
      $Flag = \{(\lambda_{new} < \lambda_{old}/\alpha)~OR~(\kappa_{itr}=\kappa)\}$;
       
      \If(\tcp*[h]{adaptively change batch/lr}){Flag}{
      $B_{itr}\asteq\beta$;~~
      $\eta_{itr}\asteq\beta$;
      $\gamma \diveq \omega$;~
      $\kappa_{itr}=0$;~
      }
      \If{$\lambda_{new} < \lambda_{old}/\alpha$}{
      $\lambda_{old}=\lambda_{new}$;
      }
      
      \If{Epoch $=\tau$ }{
        $\gamma = 0$;
      }
      \If(\tcp*[h]{lr decay schedule}){Epoch in $E_{decay}$}{
      $\eta_{itr} \diveq \rho_{lr, decay}$ ;
      }    
    }
\end{algorithm}





==> makefile <==
compilePdfOptions=
compPdftex=pdflatex ${compilePdfOptions}
compile= ${compPdftex}

TARGET=bin/main.pdf
#TARGET= bin/sigconf.pdf
MAIN=main.tex
FILES=main.tex


.SECONDEXPANSION:

####################  COMPILE PDF  ######################

all: ${TARGET}

bin/%.pdf : ${FILES} # .figs_ 
	mkdir -p bin
	#latexmk  -pvc -bibtex -pdf ${MAIN}
	${compile}  $*
	-bibtex $*
	-bibtex $*
	${compile} $*
	${compile} $*
	#${compile} $*
	mv $*.pdf $@
	#make clean
	#open ${TARGET}
	@echo Done ....!


##############  EXTERNALIZE TIKZ-FIGURES  ###############

# TIKZ_FIGS_DIR=tikz_figs
# FIGS=$(shell grep -h '[:space:]*\\inputtikz' ${TIKZ_FIGS_DIR}/figures.tex | sed '1D' | \
#   sed s'/[:space:]*\\inputtikz{\(.*\)}{/\1/' )
# FIGSPDF=$(FIGS:%=%.pdf)
# 
# .figs_ : $(FIGSPDF)
# 	date &> .figs_
# 
# ${TIKZ_FIGS_DIR}/%.pdf : $$(word 1, $$(subst -, ,$${TIKZ_FIGS_DIR}/%)).tex
# 	${compile} --jobname=${TIKZ_FIGS_DIR}/$* \
# 	  '\newcommand{\fakejobname}{${TIKZ_FIGS_DIR}/$*}\input{${TIKZ_FIGS_DIR}/figures.tex}'
# 
########################  CLEAN  ########################

cleanall: clean
	rm -r -f bin/*.pdf ${TIKZ_FIGS_DIR}/*.pdf .figs_
	cd      figs/matlab && ./clean.sh
	cd tikz_figs/matlab && ./clean.sh
	@echo Cleaned All ....! 

clean:
	rm -f *.aux *.dvi *.blg *.bbl *.out *.log */*.log */*/*.log *~ */*~ *.fdb_latexmk *.fls *.xml* *.out
	@echo Cleaned ....! 


